How to Handle Different Types of Out-of-Distribution Scenarios in Computational Argumentation? A Comprehensive and Fine-Grained Field Study

The advent of pre-trained Language Models (LMs) has markedly advanced natural language processing, but their efficacy in out-of-distribution (OOD) scenarios remains a significant challenge. Computational argumentation (CA), modeling human argumentation processes, is a field notably impacted by these challenges because complex annotation schemes and high annotation costs naturally lead to resources barely covering the multiplicity of available text sources and topics. Due to this data scarcity, generalization to data from uncovered covariant distributions is a common challenge for CA tasks like stance detection or argument classification. This work systematically assesses LMs' capabilities for such OOD scenarios. While previous work targets specific OOD types like topic shifts or OOD uniformly, we address three prevalent OOD scenarios in CA: topic shift, domain shift, and language shift. Our findings challenge the previously asserted general superiority of in-context learning (ICL) for OOD. We find that the efficacy of such learning paradigms varies with the type of OOD. Specifically, while ICL excels for domain shifts, prompt-based fine-tuning surpasses for topic shifts. To sum up, we navigate the heterogeneity of OOD scenarios in CA and empirically underscore the potential of base-sized LMs in overcoming these challenges.

==> parts/left-over.tex <==

\paragraph{Effect of Verbalizer}

Until now, results showed the effectiveness of \textit{P+FT} when automatically curating label-indicative tokens using an automatic verbalizer $v_a$.
Next, we examine the effectiveness of this verbalizer compared to a manually curated one $v_m$ (see Appendix \autoref{subsec:prompting-templates} for token-label-mappings).
Therefore, we show in \autoref{tab:verbalizer_results} the overall results for \textit{P} and \textit{P+FT} for \textit{DeBERTa-v3} in combination with $v_a$ and $v_m$ - find detailed results in the Appendix \autoref{subsec:full-manual-verbalizer}.
We note better \textit{Applicability} when using the automatic verbalizer $v_a$.
This observation is more saturated for \textit{P} than \textit{P+FT}.
Thus, we see having a more extensive set of tokens as classification proxies as beneficial to open up broad model generalization capabilities. 

\begin{table}[t]
\centering
    \setlength{\tabcolsep}{5pt}
    \resizebox{0.48\textwidth}{!}{%
        \begin{tabular}{l|cccc}
        \toprule
             & \textbf{P+\textit{$v_m$}} & \textbf{P+\textit{$v_a$}} & \textbf{P+FT+\textit{$v_m$}} & \textbf{P+FT+\textit{$v_a$}}\\
        \midrule
    \textit{\textbf{Applicability}} ($F_1$) & $34.6\pm2.8$ & $50.7\pm1.0$ &  $72.0\pm1.9$ & $72.6\pm0.8$\\
    \textit{\textbf{Reliability}} ($\tau$) & - & - & $-89.2\pm5.9$ & $-86.8\pm6.6$\\
        \bottomrule
        \end{tabular}
    }
    \caption{Comparing the overall results for the seven English-only tasks using manual ($v_m$) or automatic verbalizer ($v_a$) for \textit{P} and \textit{P+FT}.}
    \label{tab:verbalizer_results}
\end{table}



\begin{CJK}{UTF8}{min}
\begin{table}[t]
\centering
    \setlength{\tabcolsep}{3pt}
    \resizebox{0.5\textwidth}{!}{%
    \begin{tabular}{lll}
    \toprule
    &  \bf Prompt & \bf Manual Verbalizer \\
    \midrule
    arg-qua &    \pattern{ARG-1} is \pattern{MASK} than \pattern{ARG-2} regarding \pattern{TOPIC}& \makecell[l]{
        \pattern{ARG-1}: better\\
        \pattern{ARG-2}: worse
    }\\

    
    arg-sim &    \pattern{ARG-1} is \pattern{MASK} than \pattern{ARG-2} regarding \pattern{TOPIC}& \makecell[l]{
        \pattern{similar}: similar\\
        \pattern{not-similar}: different
    }\\
    
    
    arg-cls &    The attitude of \pattern{ARG} is \pattern{MASK} regarding \pattern{TOPIC}& \makecell[l]{
        \pattern{no-argument}: neutral, unrelated\\
        \pattern{pro}: for, in favor, support\\
        \pattern{con}: against, versus
    }\\
    

    evi-cls &    \pattern{TEXT} is \pattern{MASK} evidence regarding \pattern{TOPIC}& \makecell[l]{
        \pattern{evidence}: a\\
        \pattern{no-evidence}: no
    }\\ \midrule
    

    review &    The sentiment of \pattern{REVIEW} is \pattern{MASK} & \makecell[l]{
        \pattern{positive}: positive\\
        \pattern{negative}: negative
    }\\

    stance &   The attitude of \pattern{TEXT} is \pattern{MASK} regarding \pattern{TOPIC} & \makecell[l]{
        \pattern{pro}: pro, favor, for\\
        \pattern{con}: anti, against\\
        \pattern{neutral}: other, none, observing
    }\\
    entail &  \pattern{SENTENCE-1}? \pattern{MASK}, \pattern{SENTENCE-2} & \makecell[l]{
        \pattern{entailment}: yes\\
        \pattern{no-entailment}: no
    }\\ \midrule

    x-stance &   \makecell[l]{
        de: Die Haltung von \pattern{ARG} ist \pattern{MASK} zu \pattern{TOPIC} \\
        fr: L'attitude de \pattern{ARG} est \pattern{MASK} envers \pattern{TOPIC} \\
        it: L'atteggiamento di \pattern{ARG}   \pattern{MASK} verso \pattern{TOPIC}
    } & \makecell[l]{
        \pattern{pro}: pro, dafür, par, \\per questo, per, pourça \\
        \pattern{con}: kontra, dagegen, \\contro di esso, contro, contre, encontre\\
    }\\
    
    x-review &   \makecell[l]{
        de: Die Stimmung von \pattern{REVIEW} ist \pattern{MASK}\\
        en: The sentiment of \pattern{REVIEW} is \pattern{MASK} \\
        fr: Le sentiment de \pattern{REVIEW} est \pattern{MASK} \\
        jp: \pattern{REVIEW} の感情は \pattern{MASK} です
    }& \makecell[l]{
        \pattern{negative}: negativ, negative, \\négative, ネガティブ\\
        \pattern{positive}: positiv, positive, \\ネガティブ\\
    }
    \\
        \bottomrule
        \end{tabular}
    }
    \caption{Overview of the used prompt templates we use for all the proposed tasks as well as the tokens-label mapping considered for the manual verbalizer.}
    \label{tab:prompts}
\end{table}

\end{CJK}



\begin{table*}[t]
\centering
    \setlength{\tabcolsep}{5pt}
    \resizebox{1.00\textwidth}{!}{%
        \begin{tabular}{l|cccc|ccc|cc|c|c}
        \toprule
             & \bf arg-qua & \bf arg-sim & \bf arg-cls & \bf evi-cls & \bf review & \bf stance &  \bf entail & \bf x-stance & \bf x-review & \bf \multirow{2}{*}{avg. $F_1$}  & \bf \multirow{2}{*}{avg. $\rho$}\\
         &   \it  \small{Top.}   &    \it   \small{Top.}  &   \it       \small{Top.}    &   \it   \small{Top.}     &   \it  \small{Dom.}     &   \it    \small{Dom.}   &    \it     \small{Dom.}      &      \it       \small{Ling./Top.} &   \it          \small{Ling./Dom.}  &             \\
        \midrule

\textbf{P+\textit{$v_m$}}  &   34.1 &   34.6 &        20.1 &     34.4 &    38.8 &    20.4 &        35.8 &  40.4/40.1 &   41.3/36.3 &  $34.6\pm2.8$ &    - \\
\textbf{P+\textit{$v_a$}} &  54.2 &   58.6 &        40.3 &     57.2 &    61.9 &    26.5 &        44.8 &  51.1/51.2 &   54.4/52.0 &  $50.7\pm1.0$ &    - \\
\textbf{P+FT+\textit{$v_m$}}&   79.2 &   74.2 &        74.0 &     78.6 &    94.5 &    30.6 &        36.7 &  69.5/69.2 &   92.4/91.3 &  $72.0\pm1.9$ &  $-89.2\pm5.9$ \\
\textbf{P+FT+\textit{$v_a$}} &   78.5 &   79.1 &        74.6 &     78.6 &    94.2 &    33.0 &        36.7 &  69.7/69.9 &   92.6/91.4 &  $72.6\pm0.8$ &  $-86.8\pm6.6$\\
        \bottomrule
        \end{tabular}
    }
    \caption{TODO}
    \label{tab:mainresults}
\end{table*}



With these strong results of \textit{LoRA}, we examine how well \textit{P+FT} scales to bigger LMs - namely \textit{PYTHIA (2.8B)}, \textit{T5 (3B)}, and \textit{TK-Instruct (3B)}.
We note that performance does not scale for \textit{PYTHIA} but for \textit{T5} and \textit{TK-Instruct}.
We see this being due to the unidirectional encoding of \textit{PYTHIA}.
Further, we observe that instruction-based fine-tuning equips \textit{TK-Instruct} with better generalization capabilities. 
Primarily, we evaluate generalization across datasets for \textit{stance} and \textit{entail}. 
When comparing these LMs, it is important to keep in mind that the instruction-based fine-tuning of \textit{TK-Instruct} may leak semantic or task information.
These results show we can scale prompt-based fine-tuning to larger LMs with parameter-efficient methods. 

